Nowcasting Gentrification Using Airbnb Data

There is a rumbling debate over the impact of gentrification: presumed gentrifiers have been the target of protests and attacks in some cities, while they have been welcome as generators of new jobs and taxes in others. Census data fails to measure neighborhood change in real-time since it is usually updated every ten years. This work shows that Airbnb data can be used to quantify and track neighborhood changes. Specifically, we consider both structured data (e.g. number of listings, number of reviews, listing information) and unstructured data (e.g. user-generated reviews processed with natural language processing and machine learning algorithms) for three major cities, New York City (US), Los Angeles (US), and Greater London (UK). We find that Airbnb data (especially its unstructured part) appears to nowcast neighborhood gentrification, measured as changes in housing affordability and demographics. Overall, our results suggest that user-generated data from online platforms can be used to create socioeconomic indices to complement traditional measures that are less granular, not in real-time, and more costly to obtain.

==> tables/regression.tex <==
\begin{table}[ht] \centering \mytablesize
\caption{Regression for Gentrification Score.}
\begin{tabular}{
p{2.5cm}
p{2cm}
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
} 
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{City} & \multicolumn{4}{c}{Root Mean Squared Error} \\ 
\cmidrule(lr){3-6}
& & \multicolumn{1}{c}{Baseline} &
\multicolumn{1}{c}{Structured} & \multicolumn{1}{c}{Unstructured} &
\multicolumn{1}{c}{All Features}\\
\midrule
In-Sample & New York & 14.696 & 9.159 & 6.322 & 5.723 \\
Linear & Los Angeles & 15.371 & 12.187 & 6.927 & 5.628 \\
Regression & London & 17.824 & 13.716 & 12.729 & 12.087 \\
\addlinespace
\midrule
Out-of-Sample & New York & 14.356 & 9.415 & 9.877 & 9.233 \\
Random Forest & Los Angeles & 14.363 & 13.476 & 12.755 & 12.643 \\
Regression & London & 18.047 & 14.179 & 14.501 & 13.945 \\
\addlinespace
\bottomrule
\multicolumn{6}{l}{\textit{Note: Random Forest results averaged over 100 iterations with 50\%-50\% train-test split.}} \\
\end{tabular}
\label{table:regression}
\end{table}



==> tables/regression_new.tex <==
\begin{table}[ht] \centering \mytablesize
\caption{Regression: Models Without Baseline}
\begin{tabular}{
p{2cm}
p{2cm}
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
} 
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{City} & \multicolumn{5}{c}{Root Mean Squared Error} \\ 
\cmidrule(lr){3-7}
& & \multicolumn{1}{c}{Baseline: No Change} & \multicolumn{1}{c}{Baseline: Rent} &
\multicolumn{1}{c}{Structured} & \multicolumn{1}{c}{Unstructured} &
\multicolumn{1}{c}{All Features}\\
\midrule
In-Sample & New York & 14.696 & 7.829 & 9.159 & 6.322 & 5.723 \\
Linear & Los Angeles & 15.371 & 6.328 & 12.187 & 6.927 & 5.628 \\
Regression & London & 17.824 & 12.491 & 13.716 & 12.729 & 12.087 \\
\addlinespace
\midrule
Out-of-Sample & New York & 14.356 & & 9.415 & 9.877 & 9.233 \\
Random Forest & Los Angeles & 14.363 & & 13.476 & 12.755 & 12.643 \\
Regression & London & 18.047 && 14.179 & 14.501 & 13.945 \\
\addlinespace
\bottomrule
\multicolumn{6}{l}{\textit{Note: Random Forest results averaged over 100 iterations with 50\%-50\% train-test split.}} \\
\end{tabular}
\label{table:regression_new}
\end{table}


==> tables/regression_new2.tex <==
\begin{table}[ht] \centering \mytablesize
\caption{Regression: Models Include Baseline as Feature.}
\begin{tabular}{
p{2cm}
p{2cm}
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
} 
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{City} & \multicolumn{4}{c}{Root Mean Squared Error} \\ 
\cmidrule(lr){3-6}
&  & \multicolumn{1}{c}{Baseline: Rent} &
\multicolumn{1}{c}{Structured} & \multicolumn{1}{c}{Unstructured} &
\multicolumn{1}{c}{All Features}\\
\midrule
In-Sample & New York & 7.829 & 6.982 & 5.086 & 4.874 \\
Linear & Los Angeles & 6.328 & 5.267 & 3.808 & 2.495 \\
Regression & London & 12.491 & 11.766 & 10.25 & 9.964 \\
\addlinespace
\midrule
Out-of-Sample & New York  \\
Random Forest & Los Angeles  \\
Regression & London  \\
\addlinespace
\bottomrule
\multicolumn{6}{l}{\textit{Note: Random Forest results averaged over 100 iterations with 50\%-50\% train-test split.}} \\
\end{tabular}
\label{table:regression_new}
\end{table}

==> tables/regression_new3.tex <==
\begin{table}[ht] \centering \mytablesize
\caption{Sign Accuracy of Regression: Models Without Baseline}
\begin{tabular}{
p{2cm}
p{2cm}
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
} 
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{City} & \multicolumn{4}{c}{Root Mean Squared Error} \\ 
\cmidrule(lr){3-6}
&& \multicolumn{1}{c}{Baseline: Rent} &
\multicolumn{1}{c}{Structured} & \multicolumn{1}{c}{Unstructured} &
\multicolumn{1}{c}{All Features}\\
\midrule
In-Sample & New York & 75.95\% & 63.29\% & 79.75\% & 81.01\%\\
Linear & Los Angeles & 77.59\% & 72.41\% & 86.21\% & 81.03\% \\
Regression & London & 73.66\% & 67.74\% & 74.73\% & 72.58\% \\
\addlinespace
\midrule
Out-of-Sample & New York  \\
Random Forest & Los Angeles \\
Regression & London \\
\addlinespace
\bottomrule
\multicolumn{6}{l}{\textit{Note: Random Forest results averaged over 100 iterations with 50\%-50\% train-test split.}} \\
\end{tabular}
\label{table:regression_new}
\end{table}


==> tables/regression_new4.tex <==
\begin{table}[ht] \centering \mytablesize
\caption{Sign Accuracy of Regression: Models Include Baseline as Feature.}
\begin{tabular}{
p{2cm}
p{2cm}
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
S[table-number-alignment = center, group-digits=true, table-format= 2.2, group-separator={}, round-mode=places, round-precision=2]
} 
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{City} & \multicolumn{4}{c}{Root Mean Squared Error} \\ 
\cmidrule(lr){3-6}
&& \multicolumn{1}{c}{Baseline: Rent} &
\multicolumn{1}{c}{Structured} & \multicolumn{1}{c}{Unstructured} &
\multicolumn{1}{c}{All Features}\\
\midrule
In-Sample & New York & 75.95\% & 77.22\% & 84.81\% & 84.81\% \\
Linear & Los Angeles & 77.59\% & 81.03\% & 84.48\% & 86.21\% \\
Regression & London & 73.66\% & 75.27\% & 77.96\% & 78.49\% \\
\addlinespace
\midrule
Out-of-Sample & New York  \\
Random Forest & Los Angeles \\
Regression & London \\
\addlinespace
\bottomrule
\multicolumn{6}{l}{\textit{Note: Random Forest results averaged over 100 iterations with 50\%-50\% train-test split.}} \\
\end{tabular}
\label{table:regression_new}
\end{table}
